Joint Stereo Video Deblurring, Scene Flow Estimation and Moving Object Segmentation

Stereo videos for the dynamic scenes often show unpleasant blurred effects due to the camera motion and the multiple moving objects with large depth variations. Given consecutive blurred stereo video frames, we aim to recover the latent clean images, estimate the 3D scene flow and segment the multiple moving objects. These three tasks have been previously addressed separately, which fail to exploit the internal connections among these tasks and cannot achieve optimality. In this paper, we propose to jointly solve these three tasks in a unified framework by exploiting their intrinsic connections. To this end, we represent the dynamic scenes with the piece-wise planar model, which exploits the local structure of the scene and expresses various dynamic scenes. Under our model, these three tasks are naturally connected and expressed as the parameter estimation of 3D scene structure and camera motion (structure and motion for the dynamic scenes). By exploiting the blur model constraint, the moving objects and the 3D scene structure, we reach an energy minimization formulation for joint deblurring, scene flow and segmentation. We evaluate our approach extensively on both synthetic datasets and publicly available real datasets with fast-moving objects, camera motion, uncontrolled lighting conditions and shadows. Experimental results demonstrate that our method can achieve significant improvement in stereo video deblurring, scene flow estimation and moving object segmentation, over state-of-the-art methods.

==> TIP-Joint Stereo Video Deblurring, Scene Flow Estimation and Moving Objects Segmentation/experiments.tex <==
\section{Experiments}\label{sec:experiments}

To demonstrate the effectiveness of our method, we evaluate it based on two datasets: the synthetic chair sequence~\cite{sellent2016stereo} and the KITTI dataset~\cite{geiger2013vision}. We report our results on both datasets in the following sections.

%=================Table our blur model compare with others===============
\begin{table}[ht]\footnotesize
\centering
\vspace{-2 mm}
\caption{Quantitative comparisons on disparity, optical flow and deblurring results on the KITTI dataset (BlurData-1).%\MM{Liyuan: CHECK WHETHER THE SEQUENCE IS BLURDATA-1??? TOGETHER WITH THE DESCRIPTION IN THE TEXT.}. %(the best results are in bold)
}
\label{all_all}
\begin{tabular}{c|c|c|c|c|c|c|c}
\hline
\multicolumn{2}{c|}{\multirow{2}{*}{KITTI Dataset}} & \multicolumn{2}{c|}{Disparity} & \multicolumn{2}{c|}{Flow} & \multicolumn{2}{c}{PSNR} \\ \cline{3-8}
\multicolumn{2}{c|}{}                                      & m              & m+1           & Left        & Right       & Left        & Right    \\ \hline
\multicolumn{2}{c|}{\rc{Vogel} \etal ~\cite{vogel20153d}}        & 8.20           & 8.50          & 13.62       & 14.59       & /           & /        \\ \hline
\multicolumn{2}{c|}{Kim and Lee ~\cite{hyun2015generalized}}& /              & /             & 38.89       & 39.45       & 28.25       & 29.00    \\ \hline
\multicolumn{2}{c|}{Sellent \etal ~\cite{sellent2016stereo}}& 8.20           & 8.50          & 13.62       & 14.59       & 27.75       & 28.52    \\ \hline
\multicolumn{2}{c|}{\rc{Kupyn \etal ~\cite{Kupyn_2018_CVPR}}}& /           & /          & /       & /       & \rc{28.34}       & \rc{28.73}    \\ \hline
\multicolumn{2}{c|}{\rc{Tao \etal ~\cite{Tao_2018_CVPR}}}& /           & /          & /       & /       & \rc{29.55}       & \rc{29.95}    \\ \hline
\multicolumn{2}{c|}{Pan \etal~\cite{Pan_2017_CVPR}}         & 6.82           &  8.36         & 10.01        & 11.45       & 29.80       & 30.30    \\ \hline
\multicolumn{2}{c|}{Ours}                                  & \bf 6.18       &  \bf 7.49     & \bf 9.83   & \bf 11.14    & \bf 29.85       & \bf 30.50    \\ \hline
\multicolumn{8}{c}{Baseline}                \\ \hline
\multicolumn{2}{c|}{\cite{vogel20153d} and~\cite{hyun2015generalized} }     & /   & /   & 22.42  & /           & 28.11       & /        \\ \hline
%\multicolumn{2}{c|}{Ours without iteration }               & /              & /             & /           & /           & 29.57       & /        \\ \hline
\end{tabular}
\end{table}
\vspace{-2mm}
\subsection{Experimental Setup}
\noindent{\bf Initialization.} Our model in Section~\ref{sec:model} is formulated on three consecutive stereo pairs. In particular, we treat the middle frame in the left view as the reference frame. We adopt StereoSLIC~\cite{yamaguchi2013robust} to generate superpixels. Given the stereo images, we apply the approach in~\cite{geiger2011stereoscan} to obtain sparse feature correspondences. The traditional SGM~\cite{hirschmuller2008stereo} method is applied to obtain the disparity map.  We further leverage the semantic segmentation results to provide priors for motion segmentation. \rc{In particular, we applied the pre-trained model from the high-accuracy method~\cite{wu2016wider} on our blurred image.} Based on the obtained semantics, we generate a binary map ${\bf M}$ which indicates the foreground as 1 and background as 0 by grouping the estimated semantics (see Section~\ref{sec:3.2} for details.)
%The segmentation mask is obtained by
%We use approach in~\cite{wu2016wider} to get semantic segmentation masks.
The motion hypotheses are first generated using RANSAC algorithm implemented in~\cite{geiger2011stereoscan}.
% and then refined based on Eq.~(\ref{eq: refinedK}).
%In order to obtain the model parameters $\{\theta\}_{1,2,4,5,6}$ and $\{\alpha\}$, we perform block-coordinate-descent on a subset of 30 randomly selected training images, where $\theta_3 = \gamma = 250$.
Regarding the model parameters, we perform grid search on 30 reserved images. In our experiments, we fix the model parameters as \rc{$\theta_1 = 0.7$, $\theta_2 = 5.5$,  $\theta_3 =0.7$, $\gamma = 250$, $\theta_4 = 0.37$, $\theta_5 = 17$, $\lambda=0.13$, $\alpha_{1}=3.39$, $\alpha_{2}=2.5$, $\alpha_{3}=0.25$, $\theta_{r}=0.05$, $\theta_{t}= 0.1$.}

\vspace{1mm}
\noindent{\bf Evaluation metrics.} Since our method estimates the scene flow, segments moving objects and deblurs images, we thus evaluate multiple tasks separately. As for the scene flow estimation results, we evaluate both the optical flow and disparity map by the same error metric, which is by counting the number of pixels having errors more than $3$ pixels and $5\%$ of its ground-truth. We adopt the PSNR to evaluate the deblurred image sequences for left and right view separately.~We report precision (P), recall (R) and F-measure (F) for our motion segmentation results.~Those metrics are defined as:
% {\small
\begin{equation}
\begin{aligned}
P = \frac{t_p}{t_p+f_p},\;\;R = \frac{t_p}{t_p+f_n},\;\;F = \frac{2R*P}{R+P},
\end{aligned}
\end{equation}
%}
where the true positive $t_p$ represents the number of pixels that have been correctly detected as moving objects; false positive $f_p$ are defined as pixels that have been mis-detected as moving pixels; false negative $f_n$ are denoted as moving pixels that have not been detected correctly.
Thus, for each sequence, we report disparity errors for three stereo image pairs, flow errors in forward and backward directions, and PSNR values for six images, and precision, recall and F-measure for the Moving object segmentation results.

\vspace{1mm}
\noindent\textbf{Baselines.} We first compare our scene flow results with piece-wise rigid scene flow method (PRSF)~\cite{vogel20153d}, whose performance ranks as one of the top 3 approaches on KITTI optical flow benchmark~\cite{geiger2013vision}. \rc{We then compare our results with the state-of-the-art stereo deblurring approach~\cite{sellent2016stereo}, monocular deblurring approach~\cite{kim2014segmentation} and deep-learning-based deblurring approaches~\cite{Tao_2018_CVPR,Kupyn_2018_CVPR}. }We compare our moving object segmentation results with the state-of-the-art approach using sharp stereo video sequences~\cite{zhou2017moving}. In addition, we further choose NLC~\cite{faktor2014video} and FST~\cite{papazoglou2013fast} as baselines since they are more robust to occlusions, motion blur and illumination changes according to the comprehensive evaluations in~\cite{Perazzi2016}. We make the quantitative comparison of our model w/o explicitly imposing semantics priors for our flow and deblurring results in Fig~\ref{fig:err_compare}. \rc{In addition, we compare with our previous method (Pan \etal CVPR 17) that has no semantics priors. The comparison clearly shows that the performance is improved significantly with the introduction of semantics as priors.} %In Fig.~\ref{fig:adddeblurresult}(d-e) and (j-k) qualitatively show that imposing the semantics prior can lead to better flow estimation (see the first row for the flow estimation).

\vspace{1mm}
\noindent\textbf{Runtime:}
In all experiments, we simultaneously compute two directions, namely forward and backward, scene flows, restore six blurred images and segment all moving objects. Our MATLAB implementation with C++ wrappers requires a total runtime of 35 minutes for processing one scene (6 images, 3 iterations) on a single i7 core running at 3.6 GHz.

%======================================================
%=================figure compare with others (psnr and flow err)============
% \begin{figure}[!t]\begin{center}
% \includegraphics[width=0.35\textwidth]{./a_figure/i_err_compare.eps}
% \end{center}
% \vspace{-2 mm}
% \caption{The flow estimation errors for 199 scenes in the KITTI dataset. Our method clearly outperforms the monocular and stereo video deblurring methods.}
% \label{fig:err_compare}
% \end{figure}

% \begin{figure}
% \begin{center}
% \includegraphics[width=0.35\textwidth]{./a_figure/psnr_d.eps}
% \end{center}
% \vspace{-2 mm}
% \caption{The distribution of the PSNR scores for 199 scenes in the KITTI dataset(BlurData-1). The probability distribution function for each PSNR was estimated using kernel density estimation with a normal kernel function. The heavy tail of our method means larger PSNR can be achieved using our method.}
% \label{fig:psnr_compare}
% \end{figure}

 \begin{figure}[!t]\begin{center}
% \includegraphics[width=0.235\textwidth]{./a_figure/i_err_compare.eps}
\includegraphics[width=0.225\textwidth]{./a_figure/errflow.png}
\includegraphics[width=0.225\textwidth]{./a_figure/psnr_d.eps}
\end{center}
\vspace{-2.5 mm}
\caption{Left: The flow estimation errors for 199 scenes in the KITTI dataset. Our method clearly outperforms the monocular and stereo video deblurring methods. Right: The distribution of the PSNR scores for 199 scenes in the KITTI dataset(BlurData-1). The probability distribution function for each PSNR was estimated using kernel density estimation with a normal kernel function. The heavy tail of our method means larger PSNR can be achieved using our method.}
\label{fig:err_compare}\label{fig:psnr_compare}
\end{figure}

%=================figure iter===========================================
\begin{figure}[!t]
\begin{center}
\includegraphics[width=0.225\textwidth]{./a_figure/iter_psnr_our.eps}
\includegraphics[width=0.222\textwidth]{./a_figure/iter_chair.eps}
\end{center}
\vspace{-2.5 mm}
\caption{The deblurring performance of our approach with~respect to the number of iterations. (left) Our method on our dataset with the gap of 0.3 dB between the first and the last iteration. (right) Several baselines on 'Chair'.}
\label{fig:iter_psnr}
\end{figure}

\begin{figure}[!t]
\begin{center}
\begin{tabular}{ccc}
\hspace{-4 mm}
\includegraphics[width=0.155\textwidth]{./iter/sa1.pdf}
\hspace{-4 mm}
&\includegraphics[width=0.155\textwidth]{./iter/sa2.pdf}
\hspace{-4 mm}
&\includegraphics[width=0.155\textwidth]{./iter/sa3.pdf}\\
\hspace{-4 mm}
\rcs{iterations = 1}
\hspace{-4 mm}
&\rcs{iterations = 2}
\hspace{-4 mm}
&\rcs{iterations = 3}
\end{tabular}
\end{center}
\vspace{-2.5 mm}
\caption{The moving object segmentation result with respect to the number of iterations}
\label{fig:iter_seg}
\end{figure}
%===============================================

\begin{table}\footnotesize
\centering
\caption{Moving object segmentation evaluation on the KITTI dataset BlurData-1.}
\label{tab:movingComparison}
\begin{tabular}{l|c|c|c}
\hline
Methods                                    & Recall(R)     & \rc{Precision (P)}     & F-measure (F)     \\ \hline
Menze \etal~\cite{menze2015object}        & 0.7995        & 0.5841          & 0.6045            \\ \hline
Zhou \etal~\cite{zhou2017moving}          & 0.7641        & 0.6959          & 0.7284            \\ \hline
Papazoglou \etal~\cite{papazoglou2013fast} & 0.5945        & 0.3199          & 0.2938            \\ \hline
Faktor \etal~\cite{faktor2014video}        & 0.4761        & 0.3148          &  0.3339           \\ \hline
\rc{Baseline}         & \rc{0.7633}        & \rc{0.6113}          & \rc{0.6789}           \\ \hline
Our                                        & \bf 0.8520    & \bf 0.7281      & \bf 0.7426        \\ \hline
\end{tabular}
\end{table}
%================additional result==============
\begin{figure*}
\begin{center}
%\begin{small}
% \rule{\linewidth}{1cm}
% \resizebox{\textwidth}{!}{
\begin{tabular}{cccccc}
\hspace{-0.4cm}
\includegraphics[width=0.164\textwidth]{./fig_7/blur.pdf}
&\hspace{-0.45cm}
\includegraphics[width=0.164\textwidth]{./fig_7/clean.pdf}
&\hspace{-0.4cm} \includegraphics[width=0.164\textwidth]{./fig_7/i_kim.pdf}
&\hspace{-0.4cm}\includegraphics[width=0.164\textwidth]{./fig_7/i_as.pdf}
&\hspace{-0.4cm}\includegraphics[width=0.164\textwidth]{./fig_7/i_our17.pdf}
&\hspace{-0.4cm}\includegraphics[width=0.164\textwidth]{./fig_7/i_our_nos.pdf}\\%[0.1in]
\hspace{-0.4cm}
\includegraphics[width=0.164\textwidth]{./fig_7_2/blur.pdf}
&\hspace{-0.45cm}
\includegraphics[width=0.164\textwidth]{./fig_7_2/clean.pdf}
&\hspace{-0.4cm}\includegraphics[width=0.164\textwidth]{./fig_7_2/i_kim.pdf}
&\hspace{-0.4cm}\includegraphics[width=0.164\textwidth]{./fig_7_2/i_as.pdf}
&\hspace{-0.4cm}\includegraphics[width=0.164\textwidth]{./fig_7_2/i_our17.pdf}
&\hspace{-0.4cm}\includegraphics[width=0.164\textwidth]{./fig_7_2/i_our.pdf}\\%[0.1in]
\hspace{-0.4cm}
\includegraphics[width=0.164\textwidth]{./fig_7_3/blur.pdf}
&\hspace{-0.45cm}
\includegraphics[width=0.164\textwidth]{./fig_7_3/clean.pdf}
&\hspace{-0.4cm}\includegraphics[width=0.164\textwidth]{./fig_7_3/i_kim.pdf}
&\hspace{-0.4cm}\includegraphics[width=0.164\textwidth]{./fig_7_3/i_as.pdf}
&\hspace{-0.4cm}\includegraphics[width=0.164\textwidth]{./fig_7_3/i_our17.pdf}
&\hspace{-0.4cm}\includegraphics[width=0.164\textwidth]{./fig_7_3/i_our.pdf}\\
\hspace{-0.4cm}
(a) Blurred image
&\hspace{-0.45cm}(b) GT image
&\hspace{-0.4cm}(c) \rc{Kim and Lee~\cite{hyun2015generalized}}
&\hspace{-0.4cm}(d) \rc{Sellent~\etal~\cite{sellent2016stereo}}
&\hspace{-0.4cm}(e) \rc{Pan~\etal~\cite{Pan_2017_CVPR}}
&\hspace{-0.4cm}(f) \rc{Ours}\\
\hspace{-0.4cm}
\includegraphics[width=0.164\textwidth]{./fig_7/input.pdf}
&\hspace{-0.45cm}
\includegraphics[width=0.164\textwidth]{./fig_7/seg_fst.pdf}
&\hspace{-0.4cm}\includegraphics[width=0.164\textwidth]{./fig_7/seg_nlc.pdf}
&\hspace{-0.4cm}\includegraphics[width=0.164\textwidth]{./fig_7/seg_our.pdf}
&\hspace{-0.4cm}\includegraphics[width=0.164\textwidth]{./fig_7/f_our17.pdf}
&\hspace{-0.4cm}\includegraphics[width=0.164\textwidth]{./fig_7/f_our.pdf}\\%[0.1in]
\hspace{-0.4cm}
\includegraphics[width=0.164\textwidth]{./fig_7_2/input.pdf}
&\hspace{-0.45cm}
\includegraphics[width=0.164\textwidth]{./fig_7_2/seg_fst.pdf}
&\hspace{-0.4cm}\includegraphics[width=0.164\textwidth]{./fig_7_2/seg_nlc.pdf}
&\hspace{-0.4cm}\includegraphics[width=0.164\textwidth]{./fig_7_2/seg_our.pdf}
&\hspace{-0.4cm}\includegraphics[width=0.164\textwidth]{./fig_7_2/f_our17.pdf}
&\hspace{-0.4cm}\includegraphics[width=0.164\textwidth]{./fig_7_2/f_our.pdf}\\%[0.1in]
\hspace{-0.4cm}
\includegraphics[width=0.164\textwidth]{./fig_7_3/input.pdf}
&\hspace{-0.45cm}
\includegraphics[width=0.164\textwidth]{./fig_7_3/seg_fst.pdf}
&\hspace{-0.4cm}\includegraphics[width=0.164\textwidth]{./fig_7_3/seg_nlc.pdf}
&\hspace{-0.4cm}\includegraphics[width=0.164\textwidth]{./fig_7_3/seg_our.pdf}
&\hspace{-0.4cm}\includegraphics[width=0.164\textwidth]{./fig_7_3/f_our17.pdf}
&\hspace{-0.4cm}\includegraphics[width=0.164\textwidth]{./fig_7_3/f_our.pdf}\\
\hspace{-0.4cm}
(g) Initial mask
&\hspace{-0.45cm} (h) FST~\cite{papazoglou2013fast}
&\hspace{-0.4cm}(i) NLC  ~\cite{faktor2014video}
&\hspace{-0.4cm}(j) \rc{Ours}
&\hspace{-0.4cm}(k) Pan~\etal~\cite{Pan_2017_CVPR}
&\hspace{-0.4cm}(l) Ours
\end{tabular}
% }
% \vspace{-1 mm}
\caption{\rc{Qualitative comparison of our approach with baselines for deblurring, Moving object segmentation, and flow estimations. Our method use (a) blurred image and (g) Initial semantic prior from {\bf BlurData-1} as input. (b) Ground-truth latent image. (c) Deblurring results by Kim and Lee~\cite{hyun2015generalized}. (d) Stereo deblurring results by Sellent \etal~\cite{sellent2016stereo}. (e) and (f) show our deblurring results w/o imposing semantic priors, respectively; (h) Segmentation result by~\cite{papazoglou2013fast}.  (i) Segmentation result by~\cite{faktor2014video}. (j) Our segmentation result. (k) and (l) show the optical flow estimation results w/o imposing semantic priors. Best viewed in colour on the screen.}
}
\label{fig:adddeblurresult}
\end{center}
\end{figure*}

%================= fig: real data from eccv16============
\begin{figure*}
\begin{center}
\resizebox{\textwidth}{!}{
\begin{tabular}{cccc}
\includegraphics[width=0.244\textwidth]{./a_figure/realeccv16/office_b.pdf}
&\includegraphics[width=0.244\textwidth]{./fig_6/office_kim.pdf}
&\includegraphics[width=0.244\textwidth]{./fig_6/office_as.pdf}
&\includegraphics[width=0.244\textwidth]{./a_figure/realeccv16/office_db1.pdf}\\%[0.1in]
\includegraphics[width=0.244\textwidth]{./a_figure/realeccv16/toys_b.pdf}
&\includegraphics[width=0.244\textwidth]{./fig_6/toy_kim.pdf}
&\includegraphics[width=0.244\textwidth]{./fig_6/toy_as.pdf}
&\includegraphics[width=0.244\textwidth]{./fig_6/toys_db.pdf}\\%[0.1in]
% \includegraphics[width=0.215\textwidth]{./fig_5/in.pdf}
% &\includegraphics[width=0.215\textwidth]{./fig_5/kim.pdf}
% &\includegraphics[width=0.215\textwidth]{./fig_5/as.pdf}
% &\includegraphics[width=0.215\textwidth]{./fig_5/our.pdf}\\%[0.1in]
\includegraphics[width=0.244\textwidth]{./fig_5_2/image.pdf}
&\includegraphics[width=0.244\textwidth]{./fig_5_2/kim.pdf}
&\includegraphics[width=0.244\textwidth]{./fig_5_2/as.pdf}
&\includegraphics[width=0.244\textwidth]{./fig_5_2/our1.pdf}\\%[0.1in]
(a) Blurred Images 
& (b) Kim and Lee~\cite{hyun2015generalized}
& (c)  Sellent \etal ~\cite{sellent2016stereo}  
& (d) Our results\\
\end{tabular}
}
% \vspace{-2 mm}
\caption{\rc{Sample deblur results on the real image dataset from Sellent \etal~\cite{sellent2016stereo} in $1^{st}$ and $2^{nd}$ row, and average model dataset in $3^rd$ row. It shows that our 'generalized stereo deblur' model can tackle different kinds of motion blur model and get better results. Best viewed in colour on the screen.}}
\label{fig:realeccv16}
\end{center}
\end{figure*}
%=====================================================


%================= fig: real data from cai ============
\begin{figure}
\begin{center}
% \resizebox{\textwidth}{!}{
\begin{tabular}{cc}
\includegraphics[width=0.223\textwidth]{./fig_5/in.pdf}
&\includegraphics[width=0.223\textwidth]{./fig_5/kim.pdf}\\
(a) Blurred Images 
& (b) Kim and Lee~\cite{hyun2015generalized}\\
\includegraphics[width=0.223\textwidth]{./fig_5/as.pdf}
&\includegraphics[width=0.223\textwidth]{./fig_5/our.pdf}\\%[0.1in]
 (c)  Sellent \etal ~\cite{sellent2016stereo}  
& (d) Pan \etal ~\cite{Pan_2017_CVPR}\\
\includegraphics[width=0.223\textwidth]{./fig_5/tao_835.png}
&\includegraphics[width=0.223\textwidth]{./fig_5/835.png}\\
(c)  Tao \etal ~\cite{Tao_2018_CVPR}  
& (d) Our results\\
\end{tabular}
% }
% \vspace{-2 mm}
\caption{\rc{Deblurring results on our Blur dataset. (a) The blurred image. (b) Deblurring results by Kim and Lee~\cite{hyun2015generalized}. (c) Stereo deblurring results by Sellent \etal ~\cite{sellent2016stereo}. (d) Deblurring results by Pan \etal ~\cite{Pan_2017_CVPR}. (e) Deblurring results by Tao \etal~\cite{Tao_2018_CVPR}. (f) Our result. It shows that our 'generalized stereo deblur' model can get competitive result compared with the state-of-the-art deblurring methods results. Best viewed in colour on the screen.}}
\label{fig:realcai}
\end{center}
\end{figure}
%=====================================================

\vspace{-2 mm}
\subsection{Results on KITTI}
To the best of our knowledge, currently, there are no realistic benchmark datasets that provide blurred images and corresponding ground-truth deblurring and scene flow. We take advantage of the KITTI dataset~\cite{geiger2013vision} to create a synthetic {\bf blurry image dataset} on realistic scenery, which contains 199 challenging outdoor sequences. Each sequence includes 6 images ($375 \times 1242$). Our blur image dataset is generated in two different ways.
First, we follow the general practice in image deblurring and generate the blur image dataset, referred to as~{\bf BlurData-1}, using the piecewise linear 2D kernel in Eq.~\ref{eq:kimblurKernel} which is defined on the dense scene flow.  
We use method~\cite{menze2015object} to generate dense ground-truth flows. \rc{In addition, $\tau = 0.23$ and the number of frame is $N = 20$~(see Fig.~\ref{fig:pipeline} for details).}

Second, we follow the way of generating blurry image in~\cite{kim2016dynamic}, by averaging the reference image together with its neighbouring frames. In particular, we average 7 frames in total (3 on either side of the reference frame). Note that
the image sequence in KITTI, in general, has large relative motion. We therefore only choose 10 sequences to generate blurry images based on averaging, which is denoted as {\bf BlurData-2}. In the following, we report results on our generated two synthetic datasets, respectively.

%Since the KITTI benchmarking dataset does not provide dense ground-truth flow, we use a state-of-the-art scene flow method~\cite{menze2015object} to generate dense ground-truth flows. Given the dense scene flow, the blurred images are generated using the piecewise linear 2D kernel~\ref{eq:piecewiseLinearKernal}, where the frame rate is set as $\tau = 0.23$ and the number of frame is $N = 20$~(see Figure~\ref{fig:pipeline} for details). Note that Our blur generation is quite realistic and follows the general practice in image deblurring.

\vspace{1mm}
\noindent{\bf Deblurring and Scene Flow Results.} We evaluated our approach by averaging errors and PSNR scores over $m$ and $m+1$ stereo image pairs.
%\MM{Why do we only evaluate on two pairs instead of three?}
Table~\ref{all_all} shows the PSNR values, disparity errors, and flow errors averaged over 199 test sequences on {\bf BlurData-1}. Note that our method consistently outperforms all baselines. We achieve the minimum error scores of 9.83\% for optical flow and 6.18\% for the disparity in the reference view. Figure~\ref{fig:err_compare} and Figure~\ref{fig:psnr_compare} show the estimated flows and deblurring results of the KITTI stereo flow benchmark, which includes 199 scenes. Figure \ref{fig:iter_psnr} (left) shows the performance of our deblurring stage with respect to the number of iterations. While we use 5 iterations for all our experiments, our experiments indicate that only 3 iterations are sufficient in most cases to reach an optimal performance under our model. In Figure \ref{fig:adddeblurresult}, we show qualitative results.% of our method and other methods on sample sequences from our dataset.

\vspace{1mm}
\noindent{\bf Moving Object Segmentation Results.} We report the quantitative comparison of our results with the baselines in Table~\ref{tab:movingComparison}. It shows that our approach significantly outperforms the baselines by a large margin. Fig.~\ref{fig:adddeblurresult}(g-k) show the qualitative comparison of our approach with baselines. The results show that our final segmentation follows the boundary of the moving objects very well. It further demonstrates that our approach can segment the moving objects more accurately than other approaches. Therefore, we can achieve a conclusion that joint scene flow estimation, deblurring, and moving object segmentation benefit each task.

% \vspace{1mm}
% \noindent{\bf Ablation Study.}
% We make the quantitative comparison of our model w/o explicitly imposing semantics priors for our flow and deblurring results in Fig~\ref{fig:err_compare}. Our previous method (Pan CVPR17) is the one that has no semantics priors. The comparison clearly show that the performance is improved significantly with the semantics as priors. In Fig.~\ref{fig:adddeblurresult}(d-e) and (j-k) qualitatively show that imposing the semantics prior can lead to better flow estimation (see the first row for the flow estimation).  

\vspace{-2 mm}
\subsection{Results on Other Dataset}
In order to evaluate the generalization ability of our approach on different images, we use the datasets based on the 3D kernel model and average kernel model which is different from our {\bf Blurred image dataset}.
In order to compare our performance on images blurred by the 3D kernel model, we also use the data courtesy of Sellent~\cite{sellent2016stereo}.
%\footnote{Courtesy of Sellent}. 
Those sequences contain four real and four synthetic scenes and each of them have six blurred images with its sharp images. %As only the ground-truth scene flow of synthetic chair sequence is available, we can only evaluate the performance of our method quantitatively for this scene(see Table \ref{chair} for details, where the evaluation results are averaged over 4 images). (see Figure \ref{fig:realeccv16} $1^{st}$ and $2^{nd}$ rows show the performance of the result of real scene)
The synthetic sequences are blurred by the 3D kernel model and have ground-truth for those sequences. Figure \ref{fig:iter_psnr} (right) shows the performance of several baselines on synthetic dataset. This plot affirms our assumption that jointly and simultaneously solving scene flow and video deblur benefit each other. It also shows that a simple combination of two stages cannot achieve the targeted results.
For real scenes, they use real images captured with a stereo camera which moves forward very slowly and attached to a motorized rail. By averaging the frames, they obtain motion blurred images where all objects in the scene are static and the camera moves toward the scene. For these reasons, we give the semantic segmentation map as all background (see Figure \ref{fig:realeccv16} $1^{st}$ and $2^{nd}$ rows show the performance of the result of the real scene).

In Fig. \ref{fig:realeccv16}( the $3^{rd}$ and $4^{th}$ rows.), we show qualitative results of our method and other methods on sample sequences from this two datasets, where our method again achieves the best performance.

\vspace{-3 mm}
\subsection{\rc{Limitations}}
\rc{Our method is based on calibrated stereo cameras which seem sometimes not convenient for routine application. The framework may fail in the texture-less case, the scene with strong reflection or under low lighting conditions. The occlusion will also reduce the accuracy of the segmentation boundaries. Our model cannot tackle defocus blur and scenery with transparency or translucency. }
\rcs{Following the recent deblurring works such as~\cite{kim2014segmentation,gupta2010single,dai2008motion,whyte2012non}, we make the similar assumption that the intensity integral happens in colour space during the exposure time, while we are aware of several methods model the integration in the raw sensor value and consider the effects of CRFs on motion deblurring \cite{Nah_2017_CVPR,tai2013nonlinear}.
We leave these limitations as future works.}


